A Lightweight Multi-Attack CAN Intrusion Detection System on Hybrid FPGAs

Rising connectivity in vehicles is enabling new capabilities like connected autonomous driving and advanced driver assistance systems (ADAS) for improving the safety and reliability of next-generation vehicles. This increased access to in-vehicle functions compromises critical capabilities that use legacy invehicle networks like Controller Area Network (CAN), which has no inherent security or authentication mechanism. Intrusion detection and mitigation approaches, particularly using machine learning models, have shown promising results in detecting multiple attack vectors in CAN through their ability to generalise to new vectors. However, most deployments require dedicated computing units like GPUs to perform line-rate detection, consuming much higher power. In this paper, we present a lightweight multi-attack quantised machine learning model that is deployed using Xilinx's Deep Learning Processing Unit IP on a Zynq Ultrascale+ (XCZU3EG) FPGA, which is trained and validated using the public CAN Intrusion Detection dataset. The quantised model detects denial of service and fuzzing attacks with an accuracy of above 99 % and a false positive rate of 0.07%, which are comparable to the state-of-the-art techniques in the literature. The Intrusion Detection System (IDS) execution consumes just 2.0 W with software tasks running on the ECU and achieves a 25 % reduction in per-message processing latency over the state-of-the-art implementations. This deployment allows the ECU function to coexist with the IDS with minimal changes to the tasks, making it ideal for real-time IDS in in-vehicle systems.

==> archBackup.tex <==
\section{Algorithm and Architecture}\label{sec:architecture}
A tree-based reduction logic can fully exploit the inherent data-parallelism available in the reduction operation. It is the fastest way to reduce vector/vectors of scalar data points to a single value. The tree-based method restricts that the vector size has to be a power of 2. Generalizing it to any arbitrary size is a challenge. We propose a generalized tree reduction method which we realize in the FPGA hardware. 

\subsection{Algorithm}
Generalizing a tree reduction is done in two phases: a distribution phase and a merging phase. We reduce more than one vector in parallel. In the distribution phase, the vectors are split into partitions. Equal sized partitions from different vectors are grouped, laid over a reduction tree, and reduced in parallel. The reduced value from different partitions belonging to the same vector is merged either using tree nodes or a shift-and-add sequence of operations. 




Our algorithm is divided into three phases: configure phase, distribution phase and merging phase. In configure phase, configuration values are streamed on the FPGA from host. In distribution phase, a binary tree is employed, called a routing tree network. This tree is used to distribute multiple input vectors of equal but arbitrary length to route input data (encapsulating all the values of vectors) on the base level (leaf level) in a particular fashion. Finally, in merging phase, an inverted binary tree, called a merging tree network, is utilized with some additional route and accumulate logic to reduce the vectors according to target application. \par

Each node of routing tree network has a vector present on its incoming and two outgoing edges. All the nodes store two left-shift values, which are used on the incoming edge vector, to independently generate vectors for each outgoing edge. This vector distribution method leads to a particular distribution of vector-values at the base level, where each leaf carries a scalar value. 
% This particular vector distribution method applied on input vectors enable reduction through merging tree network.  

\subsubsection{Vector Distribution Method}
Vector Distribution Method is a partition-based distribution method, where vector is partitioned and then distributed at partition level. 
% First, we look at the underlying method, employed for a single vector's partition and distribution by the routing tree network and then at the distribution with multiple vectors. 
Consider we have $n$ vectors each of size $m$, each vector is denoted by $v\textsubscript{i}$ where $i = 1,2,\cdots,n$. 
We know mathematically, every number can be expressed as a sum of different powers of two. For example: 15 can be partitioned into $8\; (2^{3}),\; 4\; (2^{2}),\; 2\;(2^{1}), \;and\; 1\;(2^{0})$. Similarly, each vector is partitioned into $j$ partitions and the size of each partition being a different power of two. We denote each partition as $p\textsubscript{i}$ where $i = 1,2,\cdots,j$. 
The partitions of the vector $v\textsubscript{i}$ follows the following condition: $|p\textsubscript{i1}| > |p\textsubscript{i2}| > \cdots > |p\textsubscript{ij}|$ (here $|.|$ represents the size of the partition). 
% Moreover, atleast $n \times m$ leaves are required at the base level.  Similarly, vector of size $m$ is divided into $j$ partitions with each partition's size being a different power of two.
At the base of routing tree network, vector is organised (moving from left to right) by sorting the vector-partitions in decreasing order of size. \par
%% do I need to write in math mode

In case of multiple vectors, each vector follows the same partition method discussed in last paragraph. However, distribution at the base level of routing tree network changes with multiple vectors. For multiple vectors, partitions of same size across vectors are grouped together and then the groups are sorted in decreasing order of partition size. All applications follow this group-wise distribution method, but within the group, distribution varies with application. 


\begin{figure}
\centering
\includegraphics[scale=0.9]{figures/microExample.eps}
\caption{The figure shows the same PE structure used for a single run configurations. In part (a), two 2x2 convolutions are executed in parallel. In part (b), two 1x3 convolutions are performed over the same structure. The shift amounts are written as tuples over the routing tree nodes.}
\label{fig:sum_example}
\end{figure}

For calculating the sum of elements of a vector, within a group, partitions of $n$ vectors are placed sequentially in a particular order and this order is maintained within the other groups. In Figure \ref{fig:sum_example}, we have 2 vectors \textbf{X} and \textbf{V} each of size 7. We call their partitions of size 4, 2, and 1 as $p\textsubscript{11}$, $p\textsubscript{12}$, $p\textsubscript{13}$ for \textbf{X} and $p\textsubscript{21}$, $p\textsubscript{22}$, $p\textsubscript{23}$ for \textbf{V}. The routing tree network organises these vectors' partitions at the base level in the following manner $p\textsubscript{11}$, $p\textsubscript{21}$, $p\textsubscript{12}$, $p\textsubscript{22}$, $p\textsubscript{13}$, $p\textsubscript{23}$, meaning partitions of size 4 appear first followed by group of partition size, 2 and 1. For dot product, within a group, elements of partitions' between whom dot product has to be performed are placed alternatively and the same order is followed within the other groups as well. In Figure \ref{fig:dot_example}, we have 2 vectors \textbf{X} and \textbf{V} of size 4 and each vector has a partition of size 4. In the level lying above MUL level, we can see both 4-size partition are grouped together and elements of partitions are placed alternatively to perform multiplication followed by addition in below layers to complete dot product.
% (but alternately values needs to be distributed dot product refer fig2b and 3)
% \subsubsection{Rationale behind partition strategy}
% The strategy to partition a vector into powers of two, encapsulates the fundamental behaviour of binary tree which is merging of two nodes, therefore facilitates vector reduction.  

\subsubsection{Vector Merging Method}
In the merging tree network, partitions belonging to same vectors are merged to generate $n$ reduced values parallely. We know binary tree reductions work smoothly for even sized vectors. 
% The first $n$ nodes of the last level of merge tree contains non-interfered correct values. 
The proposed partition-based distribution strategy exploits this property by creating partition of sizes of power of 2. 
% Even with an odd size vector which will have an odd size partition, when two is raised by power 0.   
% binary tree reduction's property 
% of merging two (even number) nodes to create a single odd node. 
% Each tree node receives input over two edges, and performs reduction operation on the values. 
% Therefore, initially at first level, merging tree reduces even size partitions of distinct vectors. 
For even size partition, no interference occurs between two nodes belonging to different vectors. For odd size partition ($2^0$), however, interference occurs between nodes of different vectors. The problem of interference begins from the first level itself if a partition of size 1 exists. Although it may seem like the problem will not appear if we do not have a partition of size 1 but that is not true. Whenever the partition size is reduced to size 1 down the tree, partition becomes a candidate for interference. For instance, partitions of size $2,\,4,\,8,\,16, \cdots$ are reduced to partitions of size 1 in $1^{st},\,2^{nd},\,3^{rd},\,4^{th},\cdots$ levels, respectively. Our algorithm solves this interference problem, arising due to odd size partition, by introducing a tree tapping\footnote{Tree Tapping is used analogous to phone tapping, here it means value is read and transmitted.} technique. This tree tapping technique works by utilizing the route and accumulate logic. All the single element partitions of a level are tapped and left-shifted\eqref{shift_val} such that they align with the nodes of their corresponding vectors for addition. 

% Additionally, left-shifted levels are passed through a mask before addition to convert all nodes to zero except the nodes corresponding to partitions of size 1. A separate route and accumulate logic is employed for shifting, masking, and addition of shifted-masked level and next level. Eventually, single element partitions are converted into garbage in next levels, but ultimately, first $n$ nodes contain correct but incomplete values at the $log(|P_{i1}|)$ level. This level is added with last level's shifted-masked values in route and accumulate logic to produce final output.\par

Following a particular distribution strategy not only gives a consistent distribution, but also enables us to design hardware of the merging tree network with predictable \textit{shift values (SV)}. The shift value is calculated with the below formula, where $l$ represents levels of reduction tree, indexed with top level as 0 and increments as we move down the tree. 

\begin{equation}\label{shift_val}SV\left( {l} \right) = ({{n}} \times 2^{(log(|P_{i1}|)-l)}) \end{equation}


\subsection{Architecture}
We propose a hardware architecture made-up of two binary tree networks where the top tree executes distribution phase and the bottom tree executes the merging phase as shown in Figure \ref{fig:sum_example}. Both the trees connect at the base of the tree (leaf level). We define total leaves present at the base level as \textit{Local Compute Size (LCS)}, hence the depth/height of each tree is $log_2 (LCS)$. \par


\subsubsection{Routing Tree Network}

% The main aim of the routing tree network is to perform partition-based distribution to provide a required distribution at base level. In configure phase, each edge is configured by the host with a left-shift value. Each node receives a vector on its input edge and forwards it on the output edges by left shifting the input vector with corresponding values. To support all types of distribution, a shift register equal to the input data length is present on both edges of each node except the base level nodes. Through these shifts, on a root to leaf path, a particular vector value is routed to one of the leaves. For example, the value $v_0$ is routed to the fifth leaf in Figure~\ref{fig:sum_example} by left shifting the original vector $v_0,\cdots,v_6$, 4 times over 3 routing nodes. 

The main aim of the routing tree network is to perform partition-based distribution to provide a required distribution at base level. In configure phase, each edge is configured by the host with a left-shift value. Each node has a vector of input data length and while traversing the tree, vectors are left shifted by values present on the edges. To support all types of distribution, a register equal to the input data length is present on all nodes except the base level nodes. Through these shifts, a particular vector value is routed from the root to one of the leaves. For example, the value $v_0$ is routed to the fifth leaf in Figure~\ref{fig:sum_example} by left shifting the original vector $v_0,\cdots,v_6$, 4 times over 3 routing nodes. 
% Observe that feature maps vectors can be replicated across nodes using a shift value of 0 on both the output edges.
Using a tree network reduces the fan-out in our architecture. More precisely, for a input vector of size $m$, the fan-out reduces from $m \times LCS$ to  $2m$ between a flat and hierarchical tree-based routing.

% The host configures each routing node with shift amounts. Figure~\ref{fig:pexample} shows two-run configurations of the same architecture with different vector sizes. In part (a), since the vector of size 4 is already a power of 2, it does not need partitioning and is mapped on the leaves for reduction by merging tree network. In part (b), the feature vector $x_0, x_1, x_2$, is split into 2 partitions, $x_0,x_1$ and $x_2$ and similarly $v_0, v_1, v_2$ is partitioned. 




\subsubsection{Merging Tree Network}

The merging tree network comprises of two synchronous pipelines running in parallel. We call these two pipelines: \textit{Reduction Tree (RT)} and \textit{Route And Accumulate (RA)}. \textit{RT} pipeline implements a binary tree where each level of binary tree is realized as a pipeline stage. Each pipeline stage comprises of reduction operator between every two nodes. Values present on the input edges are stored in registers and its utilization reduces by half every stage, as we descend the tree.\par

\textit{RA} pipeline has same number of stages as the \textit{RT} pipeline where each stage has a shift, mask, and add operation unit. The pipeline taps every stage of \textit{RT} pipeline to read one-sized partitions. 
% As we have seen, tapping is necessary, because otherwise, if we wait to read them in subsequent levels, they will merge with other vector's partition of size 1 to generate distorted values. 
The tapping mechanism is carried-out by making a copy of data present in \textit{RT} pipeline in another register present in \textit{RA} pipeline. For instance, when first level's data is copied, in the same clock cycle, copied vector is shifted\eqref{shift_val} and a mask is applied(How?). In the next clock cycle, second level of reduction tree is tapped and is ready for addition with previous level's shifted-masked vector. During this same clock cycle, after addition, resultant vector is shifted\eqref{shift_val} and masked as well, to make it available in next clock cycle for addition with third level's tapped data and so on. 






% \begin{figure*}
% \centering
% \includegraphics[scale=1]{figures/example.eps}
% \caption{The figure shows the same PE structure used in two-run configurations. In part (a), two 2x2 convolutions are executed in parallel. In part (b), two 1x3 convolutions are performed over the same structure. The shift amounts are written as tuples over the routing tree nodes.}
% \label{fig:pexample}
% \end{figure*}
\begin{figure}
\centering
\includegraphics[scale=1]{figures/dotPro.eps}
\caption{Block diagram of the Processing Engine in our accelerator. The PE is made of two trees connected at the base through an array of DSP multipliers. The PE is fully pipelined to produce output every cycle.}
\label{fig:dot_example}
\end{figure}



==> relatedworks.tex <==
\section{Related Works} \label{rel_work}



==> tables/CNN.tex <==
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.5}
\begingroup
\begin{table}[h]\scriptsize
\begin{tabular}{lcccc}
\hline
                                      & \textbf{\begin{tabular}[c]{@{}c@{}}Throughput\\ GOps/Sec\end{tabular}}           & \textbf{\begin{tabular}[c]{@{}c@{}}Performance \\ Density\\ GOps/KLUTs\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Precision\\ Fixed-Point\end{tabular}}           & \textbf{\begin{tabular}[c]{@{}c@{}}Frequency\\ MHz\end{tabular}}               \\ \hline
\multicolumn{1}{l|}{\textbf{AlexNet}} & 1200                                                                             & 5.38                                                                                 & 16 bits=8,8                                                                        & 166                                                                            \\ \cline{1-1}
\multicolumn{1}{l|}{\textbf{VGG-16}}  & 1025                                                                             & 4.60                                                                                 & 16 bits=8,8                                                                        & 166                                                                            \\ \hline
                                      & \textbf{\begin{tabular}[c]{@{}c@{}}Execution\\ Kilo Cycles \\ (EC)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Memory\\ Kilo Cycles \\ (MC)\end{tabular}}        & \textbf{\begin{tabular}[c]{@{}c@{}}Theoretical\\ Kilo Cycles \\ (TC)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Pipeline \\ Rate\\ (EC+MC)/TC\end{tabular}} \\ \hline
\multicolumn{1}{l|}{\textbf{AlexNet}} & 1096                                                                             & 112                                                                                  & 856                                                                                & 1.45                                                                           \\ \cline{1-1}
\multicolumn{1}{l|}{\textbf{VGG-16}}  & 7046                                                                             & 431                                                                                  & 5149                                                                               & 1.44                                                                           \\ \hline
\end{tabular}
\caption{The table lists the Execution Cycles (EC), Memory Cycles (MC) and Theoretical Cycles (TC) required by our overlay to process various networks. The pipeline rate (PR) to process each network is also reported. }
\label{tab:scale_cnn}
\end{table}
\endgroup

==> tables/resr_utilisation.tex <==
\renewcommand{\arraystretch}{1.5}
\begin{table}[]
\centering
\begin{tabular}{cccc}
\hline
\textbf{Method}                        & \textbf{Adders}   & \textbf{Freq.(MHz)} & \textbf{Slices} \\ \hline
\multicolumn{1}{c|}{\textbf{FCBT}~\cite{zhuo2007high}}     & 2                 & 170                 & 2859            \\ \cline{1-1}
\multicolumn{1}{c|}{\textbf{DSA}~\cite{zhuo2007high}}      & 2                 & 142                 & 2215            \\ \cline{1-1}
\multicolumn{1}{c|}{\textbf{SSA}~\cite{zhuo2007high}}      & 1                 & 165                 & 1804            \\ \cline{1-1}
\multicolumn{1}{c|}{\textbf{DB}~\cite{tai2011accelerating}}       & 1                 & 188                 & 1749            \\ \cline{1-1}
\multicolumn{1}{c|}{\textbf{MFPA}~\cite{huang2012modular}}     & 5                 & 207                 & 4491            \\ \cline{1-1}
\multicolumn{1}{c|}{\textbf{AeMFPA}~\cite{huang2012modular}}   & 2                 & 204                 & 3130            \\ \cline{1-1}
\multicolumn{1}{c|}{\textbf{Ae$^2$MFPA}~\cite{huang2012modular}}   & 2                 & 144                 & 3737            \\ \cline{1-1}
\multicolumn{1}{c|}{\textbf{SBM}~\cite{tang2019resource}}      & 1                 & 278                 & 1670            \\ \cline{1-1}
\multicolumn{1}{c|}{\textbf{TreeNet}} & \textbf{36 (FxPt)} & \textbf{200}        & \textbf{5854}   \\ \hline
\end{tabular}
\caption{Table compares the slice consumption of TreeNet along the operating frequency with other works.}
\label{tab:adder-table}
\end{table}

==> tables/util_improv.tex <==
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.3}
\begin{table}[]\scriptsize
\centering
\begin{tabular}{l|cccccccccccc|}
\cline{2-13}
                                   & \multicolumn{3}{c|}{\textbf{3 x 3}} & \multicolumn{3}{c|}{\textbf{5 x 5}} & \multicolumn{3}{c|}{\textbf{7 x 7}} & \multicolumn{3}{c|}{\textbf{9 x 9}} \\ \cline{2-13} 
\multicolumn{1}{c|}{}              & LUT        & FF         & RAM       & LUT        & FF         & RAM       & LUT        & FF         & RAM       & LUT        & FF         & RAM       \\ \hline
\multicolumn{1}{|l|}{\textbf{1}}   & 2.5x       & 2.1x       & 1.3x      & 2.2x       & 2.2x       & 1.3x      & 2.4x       & 2.8x       & 1.6x      & 2.2x       & 2.6x       & 1.4x      \\
\multicolumn{1}{|l|}{\textbf{2}}   & 2.3x       & 1.9x       & 1.2x      & 1.9x       & 1.9x       & 1.2x      & 2.2x       & 2.4x       & 1.5x      & 2.0x       & 2.1x       & 1.3x      \\
\multicolumn{1}{|l|}{\textbf{4}}   & 2.0x       & 1.9x       & 0.9x      & 1.8x       & 1.9x       & 0.9x      & 2.1x       & 2.4x       & 1.2x      & 1.8x       & 1.8x       & 1.1x      \\
\multicolumn{1}{|l|}{\textbf{8}}   & 1.9x       & 2.0x       & 1.1x      & 1.9x       & 2.1x       & 1.2x      & 2.3x       & 2.3x       & 1.6x      & 2.2x       & 1.9x       & 1.5x      \\
\multicolumn{1}{|l|}{\textbf{16}}  & 2.0x       & 2.2x       & 1.2x      & 1.9x       & 2.3x       & 1.5x      & 2.4x       & 2.5x       & 2.0x      & 2.5x       & 2.3x       & 2.1x      \\
\multicolumn{1}{|l|}{\textbf{32}}  & 2.0x       & 2.3x       & 1.1x      & 1.8x       & 2.5x       & 1.5x      & 2.3x       & 2.7x       & 1.9x      & 1.7x       & 1.7x       & 2.2x      \\
\multicolumn{1}{|l|}{\textbf{64}}  & 2.2x       & 2.5x       & 1.1x      & 1.9x       & 2.7x       & 1.5x      & 2.2x       & 2.5x       & 1.9x      & 2.0x       & 2.0x       & 2.2x      \\
\multicolumn{1}{|l|}{\textbf{128}} & 2.2x       & 2.6x       & 1.1x      & 2.0x       & 2.7x       & 1.5x      & 2.2x       & 2.5x       & 1.9x      & 2.1x       & 2.2x       & 2.3x      \\
\multicolumn{1}{|l|}{\textbf{256}} & 2.3x       & 2.7x       & 1.1x      & 2.1x       & 2.7x       & 1.5x      & 2.3x       & 2.5x       & 2.0x      & 2.1x       & 2.2x       & 2.4x      \\
\multicolumn{1}{|l|}{\textbf{512}} & 2.7x       & 2.9x       & 1.1x      & 2.4x       & 2.1x       & 1.5x      & 2.6x       & 3.0x       & 2.0x      & 3.4x       & 3.3x       & 2.4x      \\ \hline
\end{tabular}
\caption{Absolute resource numbers for the presented approach.}
\end{table}

==> tables/utilization.tex <==
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.3}
\begin{table*}[]\scriptsize
\centering
\begin{tabular}{cccccccccccccl}
\multicolumn{13}{c}{\textbf{(a) Our Work}}                                                                                                                                                                                                                                                                                                           &  \\ \cline{1-13}
\multicolumn{1}{|c|}{\textbf{Replications}} & \multicolumn{3}{c|}{\textbf{3 x 3}}                                      & \multicolumn{3}{c|}{\textbf{5 x 5}}                                      & \multicolumn{3}{c|}{\textbf{7 x 7}}                                    & \multicolumn{3}{c|}{\textbf{9 x 9}}                                     &  \\ \cline{1-13}
\multicolumn{1}{|c|}{}                      & LUT                  & FF                   & \multicolumn{1}{c|}{RAM}   & LUT                  & FF                   & \multicolumn{1}{c|}{RAM}   & LUT                  & FF                   & \multicolumn{1}{c|}{RAM} & LUT                  & FF                   & \multicolumn{1}{c|}{RAM}  &  \\ \cline{2-13}
\multicolumn{1}{|c|}{1}                     & 167                  & 299                  & \multicolumn{1}{c|}{3}     & 270                  & 410                  & \multicolumn{1}{c|}{4.5}   & 327                  & 446                  & \multicolumn{1}{c|}{5}   & 459                  & 637                  & \multicolumn{1}{c|}{7}    &  \\
\multicolumn{1}{|c|}{2}                     & 195                  & 371                  & \multicolumn{1}{c|}{4}     & 324                  & 522                  & \multicolumn{1}{c|}{5.5}   & 375                  & 592                  & \multicolumn{1}{c|}{6}   & 551                  & 887                  & \multicolumn{1}{c|}{8}    &  \\
\multicolumn{1}{|c|}{4}                     & 268                  & 514                  & \multicolumn{1}{c|}{5.5}   & 417                  & 697                  & \multicolumn{1}{c|}{7.5}   & 454                  & 785                  & \multicolumn{1}{c|}{7}   & 676                  & 1272                 & \multicolumn{1}{c|}{10}   &  \\
\multicolumn{1}{|c|}{8}                     & 414                  & 798                  & \multicolumn{1}{c|}{9}     & 610                  & 1044                 & \multicolumn{1}{c|}{11}    & 653                  & 1204                 & \multicolumn{1}{c|}{11}  & 843                  & 1771                 & \multicolumn{1}{c|}{14}   &  \\
\multicolumn{1}{|c|}{16}                    & 681                  & 1363                 & \multicolumn{1}{c|}{16}    & 981                  & 1737                 & \multicolumn{1}{c|}{18}    & 1017                 & 2023                 & \multicolumn{1}{c|}{18}  & 1209                 & 2717                 & \multicolumn{1}{c|}{21}   &  \\
\multicolumn{1}{|c|}{32}                    & 1220                 & 2489                 & \multicolumn{1}{c|}{30.5}  & 1708                 & 3127                 & \multicolumn{1}{c|}{32}    & 1734                 & 3659                 & \multicolumn{1}{c|}{32}  & 2740                 & 6851                 & \multicolumn{1}{c|}{35}   &  \\
\multicolumn{1}{|c|}{64}                    & 2133                 & 4757                 & \multicolumn{1}{c|}{59}    & 3154                 & 5897                 & \multicolumn{1}{c|}{60.5}  & 3425                 & 8064                 & \multicolumn{1}{c|}{61}  & 4485                 & 11681                & \multicolumn{1}{c|}{64}   &  \\
\multicolumn{1}{|c|}{128}                   & 4392                 & 9344                 & \multicolumn{1}{c|}{116}   & 6226                 & 12100                & \multicolumn{1}{c|}{117.5} & 6839                 & 16037                & \multicolumn{1}{c|}{118} & 8458                 & 22210                & \multicolumn{1}{c|}{120}  &  \\
\multicolumn{1}{|c|}{256}                   & 8964                 & 18823                & \multicolumn{1}{c|}{229.5} & 12407                & 24716                & \multicolumn{1}{c|}{231.5} & 13722                & 32998                & \multicolumn{1}{c|}{231} & 17200                & 45615                & \multicolumn{1}{c|}{234}  &  \\
\multicolumn{1}{|c|}{512}                   & 15526                & 36308                & \multicolumn{1}{c|}{457}   & 21916                & 46210                & \multicolumn{1}{c|}{459}   & 24938                & 65388                & \multicolumn{1}{c|}{459} & 21816                & 60139                & \multicolumn{1}{c|}{462}  &  \\ \cline{1-13}
\multicolumn{1}{l}{}                        & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}     & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}      &  \\
\multicolumn{13}{c}{\textbf{(b) FPGA 2018 }}                                                                                                                                                                                                                                                                                                 &  \\ \cline{1-13}
\multicolumn{1}{|c|}{\textbf{Replications}} & \multicolumn{3}{c|}{\textbf{3 x 3}}                                      & \multicolumn{3}{c|}{\textbf{5 x 5}}                                      & \multicolumn{3}{c|}{\textbf{7 x 7}}                                    & \multicolumn{3}{c|}{\textbf{9 x 9}}                                     &  \\ \cline{1-13}
\multicolumn{1}{|c|}{}                      & LUT                  & FF                   & \multicolumn{1}{c|}{RAM}   & LUTs                 & FF                   & \multicolumn{1}{c|}{RAM}   & LUT                  & FF                   & \multicolumn{1}{c|}{RAM} & LUT                  & FF                   & \multicolumn{1}{c|}{RAM}  &  \\ \cline{2-13}
\multicolumn{1}{|c|}{1}                     & 425                  & 631                  & \multicolumn{1}{c|}{4}     & 602                  & 917                  & \multicolumn{1}{c|}{6}     & 805                  & 1278                 & \multicolumn{1}{c|}{8}   & 1040                 & 1695                 & \multicolumn{1}{c|}{10}   &  \\
\multicolumn{1}{|c|}{2}                     & 461                  & 704                  & \multicolumn{1}{c|}{5}     & 638                  & 1032                 & \multicolumn{1}{c|}{7}     & 859                  & 1428                 & \multicolumn{1}{c|}{9}   & 1107                 & 1891                 & \multicolumn{1}{c|}{11}   &  \\
\multicolumn{1}{|c|}{4}                     & 560                  & 990                  & \multicolumn{1}{c|}{5}     & 763                  & 1366                 & \multicolumn{1}{c|}{7}     & 996                  & 1952                 & \multicolumn{1}{c|}{9}   & 1264                 & 2377                 & \multicolumn{1}{c|}{11}   &  \\
\multicolumn{1}{|c|}{8}                     & 823                  & 1632                 & \multicolumn{1}{c|}{10}    & 1158                 & 2252                 & \multicolumn{1}{c|}{14}    & 1528                 & 2856                 & \multicolumn{1}{c|}{18}  & 1911                 & 3484                 & \multicolumn{1}{c|}{22}   &  \\
\multicolumn{1}{|c|}{16}                    & 1379                 & 3017                 & \multicolumn{1}{c|}{20}    & 1925                 & 4121                 & \multicolumn{1}{c|}{28}    & 2489                 & 5231                 & \multicolumn{1}{c|}{36}  & 3059                 & 6354                 & \multicolumn{1}{c|}{44}   &  \\
\multicolumn{1}{|c|}{32}                    & 2444                 & 5919                 & \multicolumn{1}{c|}{35}    & 3216                 & 8070                 & \multicolumn{1}{c|}{49}    & 3997                 & 10176                & \multicolumn{1}{c|}{63}  & 4742                 & 12284                & \multicolumn{1}{c|}{77}   &  \\
\multicolumn{1}{|c|}{64}                    & 4826                 & 11967                & \multicolumn{1}{c|}{65}    & 6265                 & 16119                & \multicolumn{1}{c|}{91}    & 7711                 & 20290                & \multicolumn{1}{c|}{117} & 9218                 & 24465                & \multicolumn{1}{c|}{143}  &  \\
\multicolumn{1}{|c|}{128}                   & 10001                & 24661                & \multicolumn{1}{c|}{130}   & 12747                & 32879                & \multicolumn{1}{c|}{182}   & 15494                & 41194                & \multicolumn{1}{c|}{234} & 18306                & 49486                & \multicolumn{1}{c|}{286}  &  \\
\multicolumn{1}{|c|}{256}                   & 20704                & 51117                & \multicolumn{1}{c|}{260}   & 26262                & 67636                & \multicolumn{1}{c|}{364}   & 31603                & 83955                & \multicolumn{1}{c|}{468} & 37062                & 100310               & \multicolumn{1}{c|}{572}  &  \\
\multicolumn{1}{|c|}{512}                   & 43360                & 106385               & \multicolumn{1}{c|}{515}   & 54097                & 100000               & \multicolumn{1}{c|}{721}   & 64928                & 200000               & \multicolumn{1}{c|}{927} & 75862                & 204114               & \multicolumn{1}{c|}{1133} &  \\ \cline{1-13}
\end{tabular}
\caption{Absolute resource numbers for the presented approach.}
\end{table*}
